Stochastic Gradient Descent under Markovian Sampling Schemes

We study a variation of vanilla stochastic gradient descent where the optimizer only has access to a Markovian sampling scheme. These schemes encompass applications that range from decentralized optimization with a random walker (token algorithms), to RL and online system identification problems. We focus on obtaining rates of convergence under the least restrictive assumptions possible on the underlying Markov chain and on the functions optimized. We first unveil the theoretical lower bound for methods that sample stochastic gradients along the path of a Markov chain, making appear a dependency in the hitting time of the underlying Markov chain. We then study Markov chain SGD (MC-SGD) under much milder regularity assumptions than prior works (e.g., no bounded gradients or domain, and infinite state spaces). We finally introduce MC-SAG, an alternative to MC-SGD with variance reduction, that only depends on the hitting time of the Markov chain, therefore obtaining a communication-efficient token algorithm.

==> macros.tex <==
\renewcommand{\aa}{\mathbf{a}}
\providecommand{\bb}{\mathbf{b}}
\providecommand{\ee}{\mathbf{e}}
\providecommand{\zz}{\mathbf{z}}
\renewcommand{\gg}{\mathbf{g}}
\providecommand{\GG}{\mathbf{G}}
\providecommand{\hh}{\mathbf{h}}
\providecommand{\ii}{\mathbf{i}}
\providecommand{\jj}{\mathbf{j}}
\providecommand{\kk}{\mathbf{k}}
\let\lll\ll
\renewcommand{\ll}{\mathbf{l}}
\providecommand{\mm}{\mathbf{m}}
\providecommand{\nn}{\mathbf{n}}
\providecommand{\oo}{\mathbf{o}}
\providecommand{\pp}{\mathbf{p}}
\providecommand{\qq}{\mathbf{q}}
\providecommand{\rr}{\mathbf{r}}
\providecommand{\ss}{\mathbb{s}}
\providecommand{\tt}{\mathbf{t}}
\providecommand{\uu}{u}
\providecommand{\vv}{v}
\providecommand{\ww}{\beta}
\providecommand{\xx}{\mathbf{x}}
\providecommand{\yy}{\mathbf{y}}
\providecommand{\YY}{\mathbf{Y}}
\providecommand{\XX}{\mathbf{X}}
\renewcommand{\th}{\bm{\theta}}
\providecommand{\ph}{{\phi}}
\providecommand{\bt}{\bm{\beta}}
\providecommand{\ddelta}{\delta}
\renewcommand{\alph}{\alpha}


\newcommand{\E}{\mathbb{E}}




\newcommand{\cI}{\mathcal{I}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cO}{\mathcal O}
\newcommand{\mB}{\mathbf{B}}
\newcommand{\mH}{\mathbf{H}}
\newcommand{\mI}{\mathbf{I}}
\newcommand{\mJ}{\mathbf{J}}
\newcommand{\R}{\mathbb R}

\newcommand{\cE}{\mathcal{E}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\sparse}{{\rm sparse}}
\newcommand{\Gain}{{\rm Gain}}
\renewcommand{\empty}{\varnothing}

\newcommand{\eqdef}{\stackrel{\text{def}}{=}}
\newcommand{\avein}{\frac{1}{n}\sum_{i=1}^n}

\newcommand{\lr}[1]{\langle #1\rangle}
\DeclareMathOperator{\prox}{prox}
\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\id}{Id}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator{\Ima}{Im}
\DeclareMathOperator{\argsinh}{arcsinh}
\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\clconv}{\overline{conv}}
\def\<#1,#2>{\langle #1,#2\rangle}
\newcommand{\sumin}{\sum \limits_{i=1}^n}
\newcommand{\sumjn}{\sum \limits_{j=1}^n}


\definecolor{myblue}{RGB}{55,126,184}
\newcommand{\bluebox}[1]{\colorbox{myblue!30}{#1}}


\newcommand{\GD}{{\rm GD}}
\newcommand{\SGD}{{\rm SGD}}

\usepackage{dsfont}



\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\le}{\leqslant}
\renewcommand{\ge}{\geqslant}

\def\<{\langle}
\def\>{\rangle}
\def\|{\Vert}

\definecolor{NavyBlue}{rgb}{0.1,0.1,0.6}
\newcommand{\mathieu}[1]{{\color{blue} ME: #1}}
\newcommand{\Snote}[1]{{\color{olive} Scott: #1}}
\newcommand{\sg}[1]{{\color{red} SG: #1}}
\newcommand{\note}[1]{{\color{brown} \textbf{Note:} #1}}

\def\bfone{{\boldsymbol 1}}
\def\eps{\varepsilon}
\def\var{{\rm var\,}}


\newcommand{\comm}{{\rm comm}}
\newcommand{\comp}{{\rm comp}}
\newcommand{\rel}{{\rm rel}}
\newcommand{\gitilde}{\tilde{g}^*_i}
\newcommand{\esp}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\espk}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\NRM}[1]{{{\left\| #1\right\|}}} % ||1||% Operators
\newcommand{\set}[1]{{{\left\{ #1\right\}}}} % ||1||% Operators
\newcommand{\proba}[1]{\mathbb{P}\left(#1\right)}


\newcommand{\gau}[1]{\mathcal{N}(0, #1)}
\newcommand{\Gau}[1]{\mathcal{N}(0, #1 I)}
\newcommand{\Obs}[1]{\mathcal{O}_{#1}}


\newcommand{\half}{\frac{1}{2}}

% \usepackage{enumerate}
% \setlist[enumerate]{itemsep=0mm}

\newcommand{\D}{\mathbb{D}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\tq}{\tilde{q}}
\newcommand{\balpha}{{\bm{\alpha}}}

\newcommand{\dd}{{\rm d}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cH}{\mathcal{H}}

\newcommand{\N}{\mathbb{N}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\Ker}{{\rm Ker}}
\newcommand{\cons}{{\rm cons}}
\newcommand{\out}{{\rm out}}
\newcommand{\xit}{{\xi_t}}

% from Radu
\newcommand{\interior}{{ \rm int}\ }
\newcommand{\reals}{\R}
\newcommand{\support}{{\rm supp}}

\hypersetup{colorlinks=true, urlcolor= blue, linkcolor=blue, citecolor=blue}





\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{amscd}
\usepackage{caption}
%\usepackage{subcaption}
\usepackage{indentfirst}
\usepackage{cleveref}
\usepackage{mathtools}
\usepackage{thmtools} 
\usepackage{thm-restate}
\usepackage{bm}
\usepackage{multicol}
\usepackage{wrapfig}

% Use \Name{Author Name} to specify the name.
% If the surname contains spaces, enclose the surname
% in braces, e.g. \Name{John {Smith Jones}} similarly
% if the name has a "von" part, e.g \Name{Jane {de Winter}}.
% If the first letter in the forenames is a diacritic
% enclose the diacritic in braces, e.g. \Name{{\'E}louise Smith}

% Two authors with the same address
% \coltauthor{\Name{Author Name1} \Email{abc@sample.com}\and
%  \Name{Author Name2} \Email{xyz@sample.com}\\
%  \addr Address}

% Three or more authors with the same address:
% \coltauthor{\Name{Author Name1} \Email{an1@sample.com}\\
%  \Name{Author Name2} \Email{an2@sample.com}\\
%  \Name{Author Name3} \Email{an3@sample.com}\\
%  \addr Address}

% Authors with different addresses:


\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\ext}{ext}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\esssup}{ess\,sup}




\newcommand{\edgeuv}{{\{u,v\}}}
\newcommand{\edgevw}{{\{v,w\}}}
\newcommand{\edgeuw}{{\{u,w\}}}
\newcommand{\edgevtwt}{{\{v_t,w_t\}}}

\newcommand{\utov}{{u\to v}}
\newcommand{\utow}{{u\to w}}
\newcommand{\vtow}{{v\to w}}

\newcommand{\mix}{{\rm mix}}
\newcommand{\hit}{{\rm hit}}
\newcommand{\cov}{{\rm cov}}

\newcommand{\Authornote}[2]{{\sffamily\small\color{red}{[#1: #2]}}}
\newcommand{\nf}{\Authornote{N}}
% \newcommand{\Snote}{\Authornote{S}}


\newtheorem{theorem}{Theorem}
\newtheorem{theoreminformal}{Theorem}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}
%\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{corollary}{Corollary}
\crefname{assumption}{assumption}{assumptions}

